Optimized explicit Runge-Kutta schemes for the spectral difference method applied to wave propagation problems

Explicit Runge-Kutta schemes with large stable step sizes are developed for integration of high order spectral difference spatial discretization on quadrilateral grids. The new schemes permit an effective time step that is substantially larger than the maximum admissible time step of standard explicit Runge-Kutta schemes available in literature. Furthermore, they have a small principal error norm and admit a low-storage implementation. The advantages of the new schemes are demonstrated through application to the Euler equations and the linearized Euler equations.

==> tables/efficiencies/table-efficiency-comparison-annulus-selected-optimal-erk2.tex <==
\begin{table}
\centering
\begin{tabular}{c|c|c|c}  
Method & {$s$} & {$\chi^{stab}$} & $CPU time ratio$  \\ \hline
Midpoint ERK(2,2) & {\em 2}& {\em 1} & {\em 1} & \\ \hline 
Optimal ERK(3,2) & {3} &{1.11} & 1.10  \\ 
Optimal ERK(8,2) & {8} &{1.19} & 1.18\\ 
\end{tabular} 
\caption{Theoretical and observed stability efficiency of the selected optimal
2$^\mathrm{nd}$-order ERK methods.  The reference 2-stage method (corresponding to the
values in italics) is the midpoint ERK method.
\label{tab:efficiencies-comparison-selected-optimal-erk2}}
\end{table} 



==> tables/efficiencies/table-efficiency-comparison-annulus-selected-optimal-erk3.tex <==
\begin{table}
\centering
\begin{tabular}{c|c|c|c}  
Method & {$s$} & {$\chi^{stab}$} & $CPU time ratio$  \\ \hline
Heun's ERK(3,3) & {\em 3}& {\em 1} & {\em 1} & \\ \hline 
Optimal ERK(5,3) & {3} &{1.20} & 1.20  \\ 
Optimal ERK(17,3) & {8} &{1.42} & 1.42\\ 
\end{tabular} 
\caption{Theoretical and observed stability efficiency of the selected optimal
3$^\mathrm{rd}$-order ERK methods.  The reference method (corresponding to the values in italics) is Heun's 3-stage method.
\label{tab:efficiencies-comparison-selected-optimal-erk3}}
\end{table}


==> tables/efficiencies/table-efficiency-optimal-erk2.tex <==
\begin{table}
\centering
\begin{tabular}{ccc|c|c} 
& & &\multicolumn{2}{c}{Comparison with ERK(2,2)}\\ \hline 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & &\\ 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & & $\chi^{stab}$ & $\chi^{acc}$ \\ 
\multicolumn{1}{c|}{$s$} & \multicolumn{1}{c|}{$H/s$} & $C^{(p+1)}$ & $(H/s)_{ERK(2,2)}$ = 1.7678e-01 & $(C)^{(p+1)}_{ERK(2,2)}$ = 1.7180e-01\\ 
\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & & & \\ \hline 
\multicolumn{1}{c|}{3} &\multicolumn{1}{c|}{1.9587e-01} & 7.5938e-02 & 1.11 & 1.00 \\ 
\multicolumn{1}{c|}{4} &\multicolumn{1}{c|}{2.0429e-01} & 4.2924e-02 & 1.16 & 1.00 \\ 
\multicolumn{1}{c|}{5} &\multicolumn{1}{c|}{2.0692e-01} & 2.7899e-02 & 1.17 & 0.99 \\ 
\multicolumn{1}{c|}{6} &\multicolumn{1}{c|}{2.0852e-01} & 1.9662e-02 & 1.18 & 0.99 \\ 
\multicolumn{1}{c|}{7} &\multicolumn{1}{c|}{2.0925e-01} & 1.4666e-02 & 1.18 & 0.98 \\ 
\multicolumn{1}{c|}{8} &\multicolumn{1}{c|}{2.0968e-01} & 1.1294e-02 & 1.19 & 0.98 \\ 
\multicolumn{1}{c|}{9} &\multicolumn{1}{c|}{2.0991e-01} & 8.9584e-03 & 1.19 & 0.97 \\ 
\multicolumn{1}{c|}{10} &\multicolumn{1}{c|}{2.1006e-01} & 7.2938e-03 & 1.19 & 0.97 \\ 
\multicolumn{1}{c|}{11} &\multicolumn{1}{c|}{2.1015e-01} & 6.0554e-03 & 1.19 & 0.97 \\ 
\multicolumn{1}{c|}{12} &\multicolumn{1}{c|}{2.1020e-01} & 5.1054e-03 & 1.19 & 0.97 \\ 
\multicolumn{1}{c|}{13} &\multicolumn{1}{c|}{2.1023e-01} & 4.3536e-03 & 1.19 & 0.97 \\ 
\multicolumn{1}{c|}{14} &\multicolumn{1}{c|}{2.1024e-01} & 3.7598e-03 & 1.19 & 0.97 \\ 
\multicolumn{1}{c|}{15} &\multicolumn{1}{c|}{2.1026e-01} & 3.2777e-03 & 1.19 & 0.97 \\ 
\multicolumn{1}{c|}{16} &\multicolumn{1}{c|}{2.1027e-01} & 2.8846e-03 & 1.19 & 0.96 \\ 
\multicolumn{1}{c|}{17} &\multicolumn{1}{c|}{2.1027e-01} & 2.5555e-03 & 1.19 & 0.96 \\ 
\multicolumn{1}{c|}{18} &\multicolumn{1}{c|}{2.1028e-01} & 2.2803e-03 & 1.19 & 0.96 \\ 
\multicolumn{1}{c|}{19} &\multicolumn{1}{c|}{2.1028e-01} & 2.0476e-03 & 1.19 & 0.96 \\ 
\multicolumn{1}{c|}{20} &\multicolumn{1}{c|}{2.1028e-01} & 1.8480e-03 & 1.19 & 0.96 \\ 
\hline 
\end{tabular} 
\caption{Step size, stability efficiency $\chi^{(stab)}$ and estimation of global accuracy efficiency $\chi^{(acc)}$ of the optimized second-order explicit Runge--Kutta methods. 
\label{tab:efficiencies-optimal-erk2}
\end{table} 


==> tables/efficiencies/table-efficiency-optimal-erk3.tex <==
\begin{table}
\centering
\begin{tabular}{ccc|c|c} 
& & &\multicolumn{2}{c}{Comparison with ERK(3,3)}\\ \hline 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & &\\ 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & & $\chi^{stab}$ & $\chi^{acc}$ \\ 
\multicolumn{1}{c|}{$s$} & \multicolumn{1}{c|}{$H/s$} & $C^{(p+1)}$ & $(H/s)_{ERK(3,3)}$ = 7.5739e-02 & $(C)^{(p+1)}_{ERK(3,3)}$ = 4.6296e-02\\ 
\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & & & \\ \hline 
\multicolumn{1}{c|}{4} &\multicolumn{1}{c|}{8.3650e-02} & 1.6861e-02 & 1.10 & 1.05 \\ 
\multicolumn{1}{c|}{5} &\multicolumn{1}{c|}{9.0719e-02} & 9.9290e-03 & 1.20 & 1.00 \\ 
\multicolumn{1}{c|}{6} &\multicolumn{1}{c|}{9.5469e-02} & 6.5845e-03 & 1.26 & 0.96 \\ 
\multicolumn{1}{c|}{7} &\multicolumn{1}{c|}{9.8790e-02} & 4.6378e-03 & 1.30 & 0.92 \\ 
\multicolumn{1}{c|}{8} &\multicolumn{1}{c|}{1.0104e-01} & 3.5119e-03 & 1.33 & 0.89 \\ 
\multicolumn{1}{c|}{9} &\multicolumn{1}{c|}{1.0270e-01} & 2.7366e-03 & 1.36 & 0.86 \\ 
\multicolumn{1}{c|}{10} &\multicolumn{1}{c|}{1.0390e-01} & 2.2000e-03 & 1.37 & 0.83 \\ 
\multicolumn{1}{c|}{11} &\multicolumn{1}{c|}{1.0477e-01} & 1.7963e-03 & 1.38 & 0.81 \\ 
\multicolumn{1}{c|}{12} &\multicolumn{1}{c|}{1.0544e-01} & 1.4825e-03 & 1.39 & 0.79 \\ 
\multicolumn{1}{c|}{13} &\multicolumn{1}{c|}{1.0599e-01} & 1.2473e-03 & 1.40 & 0.77 \\ 
\multicolumn{1}{c|}{14} &\multicolumn{1}{c|}{1.0638e-01} & 1.0792e-03 & 1.40 & 0.75 \\ 
\multicolumn{1}{c|}{15} &\multicolumn{1}{c|}{1.0670e-01} & 9.2760e-04 & 1.41 & 0.74 \\ 
\multicolumn{1}{c|}{16} &\multicolumn{1}{c|}{1.0698e-01} & 8.0282e-04 & 1.41 & 0.72 \\ 
\multicolumn{1}{c|}{17} &\multicolumn{1}{c|}{1.0718e-01} & 7.1115e-04 & 1.42 & 0.71 \\ 
\multicolumn{1}{c|}{18} &\multicolumn{1}{c|}{1.0737e-01} & 6.2741e-04 & 1.42 & 0.70 \\ 
\multicolumn{1}{c|}{19} &\multicolumn{1}{c|}{1.0752e-01} & 5.6291e-04 & 1.42 & 0.69 \\ 
\multicolumn{1}{c|}{20} &\multicolumn{1}{c|}{1.0765e-01} & 5.0234e-04 & 1.42 & 0.68 \\ 
\hline 
\end{tabular} 
\caption{Step size, stability efficiency $\chi^{(stab)}$ and estimation of global accuracy efficiency $\chi^{(acc)}$ of the optimized third-order explicit Runge--Kutta methods. 
\label{tab:efficiencies-optimal-erk3}
\end{table} 


==> tables/efficiencies/table-efficiency-optimal-erk4.tex <==
\begin{table}
\centering
\begin{tabular}{ccc|c|c} 
& & &\multicolumn{2}{c}{Comparison with ERK(4,4)}\\ \hline 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & &\\ 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & & $\chi^{stab}$ & $\chi^{acc}$ \\ 
\multicolumn{1}{c|}{$s$} & \multicolumn{1}{c|}{$H/s$} & $C^{(p+1)}$ & $(H/s)_{ERK(4,4)}$ = 3.9534e-02 & $(C)^{(p+1)}_{ERK(4,4)}$ = 1.4505e-02\\ 
\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & & & \\ \hline 
\multicolumn{1}{c|}{5} &\multicolumn{1}{c|}{4.7333e-02} & 3.6463e-03 & 1.20 & 1.13 \\ 
\multicolumn{1}{c|}{6} &\multicolumn{1}{c|}{5.0342e-02} & 1.5121e-03 & 1.27 & 1.17 \\ 
\multicolumn{1}{c|}{7} &\multicolumn{1}{c|}{5.2841e-02} & 9.5769e-04 & 1.34 & 1.13 \\ 
\multicolumn{1}{c|}{8} &\multicolumn{1}{c|}{5.5040e-02} & 6.7529e-04 & 1.39 & 1.08 \\ 
\multicolumn{1}{c|}{9} &\multicolumn{1}{c|}{5.6977e-02} & 5.0640e-04 & 1.44 & 1.03 \\ 
\multicolumn{1}{c|}{10} &\multicolumn{1}{c|}{5.8595e-02} & 3.9517e-04 & 1.48 & 0.98 \\ 
\multicolumn{1}{c|}{11} &\multicolumn{1}{c|}{5.9998e-02} & 3.1689e-04 & 1.52 & 0.95 \\ 
\multicolumn{1}{c|}{12} &\multicolumn{1}{c|}{6.1179e-02} & 2.6334e-04 & 1.55 & 0.91 \\ 
\multicolumn{1}{c|}{13} &\multicolumn{1}{c|}{6.2173e-02} & 2.1896e-04 & 1.57 & 0.88 \\ 
\multicolumn{1}{c|}{14} &\multicolumn{1}{c|}{6.3005e-02} & 1.8975e-04 & 1.59 & 0.84 \\ 
\multicolumn{1}{c|}{15} &\multicolumn{1}{c|}{6.3718e-02} & 1.6534e-04 & 1.61 & 0.82 \\ 
\multicolumn{1}{c|}{16} &\multicolumn{1}{c|}{6.4320e-02} & 1.4236e-04 & 1.63 & 0.79 \\ 
\multicolumn{1}{c|}{17} &\multicolumn{1}{c|}{6.4798e-02} & 1.2770e-04 & 1.64 & 0.77 \\ 
\multicolumn{1}{c|}{18} &\multicolumn{1}{c|}{6.5233e-02} & 1.1087e-04 & 1.65 & 0.75 \\ 
\multicolumn{1}{c|}{19} &\multicolumn{1}{c|}{6.5603e-02} & 9.9896e-05 & 1.66 & 0.73 \\ 
\multicolumn{1}{c|}{20} &\multicolumn{1}{c|}{6.5931e-02} & 9.1888e-05 & 1.67 & 0.71 \\ 
\hline 
\end{tabular} 
\caption{Step size, stability efficiency $\chi^{(stab)}$ and estimation of global accuracy efficiency $\chi^{(acc)}$ of the optimized fourth-order explicit Runge--Kutta methods. 
\label{tab:efficiencies-optimal-erk4}
\end{table} 


==> tables/efficiencies/table-efficiency-optimal-erk5.tex <==
\begin{table}
\centering
\begin{tabular}{ccc|c|c} 
& & &\multicolumn{2}{c}{Comparison with ERKF(6,5)}\\ \hline 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & &\\ 
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & & $\chi^{stab}$ & $\chi^{acc}$ \\ 
\multicolumn{1}{c|}{$s$} & \multicolumn{1}{c|}{$H/s$} & $C^{(p+1)}$ & $(H/s)_{ERKF(6,5)}$ = 2.6916e-02 & $(C)^{(p+1)}_{ERKF(6,5)}$ = 3.3557e-03\\ 
\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{} & & & \\ \hline 
\multicolumn{1}{c|}{7} &\multicolumn{1}{c|}{3.3161e-02} & 7.0158e-04 & 1.23 & 1.17 \\ 
\multicolumn{1}{c|}{8} &\multicolumn{1}{c|}{3.4255e-02} & 2.4076e-04 & 1.27 & 1.27 \\ 
\multicolumn{1}{c|}{9} &\multicolumn{1}{c|}{3.5278e-02} & 1.0203e-04 & 1.31 & 1.34 \\ 
\multicolumn{1}{c|}{10} &\multicolumn{1}{c|}{3.6164e-02} & 5.0975e-05 & 1.34 & 1.39 \\ 
\multicolumn{1}{c|}{11} &\multicolumn{1}{c|}{3.6945e-02} & 2.6735e-05 & 1.37 & 1.43 \\ 
\multicolumn{1}{c|}{12} &\multicolumn{1}{c|}{3.7623e-02} & 1.6962e-05 & 1.40 & 1.44 \\ 
\multicolumn{1}{c|}{13} &\multicolumn{1}{c|}{3.8277e-02} & 1.9898e-04 & 1.42 & 0.81 \\ 
\multicolumn{1}{c|}{14} &\multicolumn{1}{c|}{3.8990e-02} & 1.3542e-05 & 1.45 & 1.29 \\ 
\multicolumn{1}{c|}{15} &\multicolumn{1}{c|}{3.9726e-02} & 1.7393e-05 & 1.48 & 1.15 \\ 
\multicolumn{1}{c|}{16} &\multicolumn{1}{c|}{4.0391e-02} & 4.0533e-05 & 1.50 & 0.91 \\ 
\multicolumn{1}{c|}{17} &\multicolumn{1}{c|}{4.0984e-02} & 6.5138e-05 & 1.52 & 0.78 \\ 
\multicolumn{1}{c|}{18} &\multicolumn{1}{c|}{4.1471e-02} & 3.2341e-05 & 1.54 & 0.84 \\ 
\multicolumn{1}{c|}{19} &\multicolumn{1}{c|}{4.1870e-02} & 2.9207e-05 & 1.56 & 0.82 \\ 
\multicolumn{1}{c|}{20} &\multicolumn{1}{c|}{4.2195e-02} & 1.0490e-05 & 1.57 & 0.95 \\ 
\multicolumn{1}{c|}{21} &\multicolumn{1}{c|}{4.2478e-02} & 2.6704e-02 & 1.58 & 0.19 \\ 
\multicolumn{1}{c|}{22} &\multicolumn{1}{c|}{4.2707e-02} & 5.9250e-03 & 1.59 & 0.24 \\ 
\hline 
\end{tabular} 
\caption{Step size, stability efficiency $\chi^{(stab)}$ and estimation of global accuracy efficiency $\chi^{(acc)}$ of the optimized fifth-order explicit Runge--Kutta methods. 
\label{tab:efficiencies-optimal-erk5}
\end{table} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk2-0.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 3 & 4 & 5 & 6 & 7 & 8 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 9.07289947e-02  & 1.23742214e-01  & 1.38767722e-01  & 1.47005053e-01  & 1.52000901e-01  & 1.55372692e-01  \\ 
  &   & 1.34936002e-02  & 2.15207262e-02  & 2.66934134e-02  & 3.00849551e-02  & 3.24812706e-02  \\ 
  &   &   & 1.49569300e-03  & 2.81954585e-03  & 3.85032588e-03  & 4.64521630e-03  \\ 
  &   &   &   & 1.37183528e-04  & 2.95258287e-04  & 4.43022755e-04  \\ 
  &   &   &   &   & 1.05605098e-05  & 2.57976940e-05  \\ 
  &   &   &   &   &   & 7.07975554e-07  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal second order explicit RK methods for $s=[3, 4, 5, 6, 7, 8]$}
\label{tbl:stab-coeffs-optimal-erk2-0}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk2-1.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 9 & 10 & 11 & 12 & 13 & 14 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 1.57708271e-01  & 1.59372818e-01  & 1.60611298e-01  & 1.61561288e-01  & 1.62313108e-01  & 1.62906855e-01  \\ 
  & 3.42082968e-02  & 3.54872104e-02  & 3.64638580e-02  & 3.72275600e-02  & 3.78392498e-02  & 3.83312025e-02  \\ 
  & 5.25660750e-03  & 5.73113558e-03  & 6.10621138e-03  & 6.40741104e-03  & 6.65331545e-03  & 6.85511988e-03  \\ 
  & 5.70526196e-04  & 6.77527812e-04  & 7.66880349e-04  & 8.41645992e-04  & 9.04593240e-04  & 9.57670844e-04  \\ 
  & 4.21524002e-05  & 5.78080022e-05  & 7.20908163e-05  & 8.48275347e-05  & 9.60715276e-05  & 1.05924585e-04  \\ 
  & 1.92768364e-06  & 3.40763815e-06  & 4.96780318e-06  & 6.50335133e-06  & 7.95917477e-06  & 9.30720580e-06  \\ 
  & 4.18532468e-08  & 1.25588609e-07  & 2.39139902e-07  & 3.69792471e-07  & 5.07703391e-07  & 6.45940107e-07  \\ 
  &   & 2.20995099e-09  & 7.25273957e-09  & 1.48150554e-08  & 2.42396616e-08  & 3.48454214e-08  \\ 
  &   &   & 1.05484062e-10  & 3.76221206e-10  & 8.20969398e-10  & 1.41719213e-09  \\ 
  &   &   &   & 4.59794842e-12  & 1.77116102e-11  & 4.11151854e-11  \\ 
  &   &   &   &   & 1.84446204e-13  & 7.62909214e-13  \\ 
  &   &   &   &   &   & 6.85085680e-15  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal second order explicit RK methods for $s=[9, 10, 11, 12, 13, 14]$}
\label{tbl:stab-coeffs-optimal-erk2-1}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk2-2.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 15 & 16 & 17 & 18 & 19 & 20 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 1.63388957e-01  & 1.63782114e-01  & 1.64111205e-01  & 1.64386317e-01  & 1.64619090e-01  & 1.64818633e-01  \\ 
  & 3.87354082e-02  & 3.90695667e-02  & 3.93510415e-02  & 3.95888794e-02  & 3.97918321e-02  & 3.99667934e-02  \\ 
  & 7.02326080e-03  & 7.16428137e-03  & 7.28420979e-03  & 7.38661600e-03  & 7.47480102e-03  & 7.55136016e-03  \\ 
  & 1.00281084e-03  & 1.04137842e-03  & 1.07464512e-03  & 1.10343058e-03  & 1.12850407e-03  & 1.15047909e-03  \\ 
  & 1.14558783e-04  & 1.22125223e-04  & 1.28785073e-04  & 1.34651276e-04  & 1.39839322e-04  & 1.44445018e-04  \\ 
  & 1.05401225e-05  & 1.16589961e-05  & 1.26719298e-05  & 1.35858196e-05  & 1.44106301e-05  & 1.51555626e-05  \\ 
  & 7.80246156e-07  & 9.08121826e-07  & 1.02842973e-06  & 1.14051244e-06  & 1.24442354e-06  & 1.34042545e-06  \\ 
  & 4.60673793e-08  & 5.74794743e-08  & 6.87897176e-08  & 7.97848574e-08  & 9.03437647e-08  & 1.00391526e-07  \\ 
  & 2.13020406e-09  & 2.92442550e-09  & 3.76891020e-09  & 4.63742262e-09  & 5.51068187e-09  & 6.37397744e-09  \\ 
  & 7.47046854e-11  & 1.17250942e-10  & 1.67043896e-10  & 2.22230533e-10  & 2.81143944e-10  & 3.42313816e-10  \\ 
  & 1.87739431e-12  & 3.58279382e-12  & 5.86433695e-12  & 8.66063762e-12  & 1.18898437e-11  & 1.54615092e-11  \\ 
  & 3.02791388e-14  & 7.87554599e-14  & 1.57553291e-13  & 2.68499464e-13  & 4.10752539e-13  & 5.81552084e-13  \\ 
  & 2.36866968e-16  & 1.11424630e-15  & 3.05499085e-15  & 6.39265825e-15  & 1.13300368e-14  & 1.79364009e-14  \\ 
  &   & 7.66117603e-18  & 3.82222978e-17  & 1.10157516e-16  & 2.40736213e-16  & 4.43105104e-16  \\ 
  &   &   & 2.32795654e-19  & 1.22746899e-18  & 3.71115933e-18  & 8.45432270e-18  \\ 
  &   &   &   & 6.66818635e-21  & 3.70655340e-20  & 1.17284156e-19  \\ 
  &   &   &   &   & 1.80725774e-22  & 1.05590079e-21  \\ 
  &   &   &   &   &   & 4.64645570e-24  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal second order explicit RK methods for $s=[15, 16, 17, 18, 19, 20]$}
\label{tbl:stab-coeffs-optimal-erk2-2}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk3-0.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 4 & 5 & 6 & 7 & 8 & 9 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 2.48053176e-02  & 3.17376770e-02  & 3.50821680e-02  & 3.70288399e-02  & 3.81547427e-02  & 3.89300493e-02  \\ 
  &   & 2.74773334e-03  & 4.37031944e-03  & 5.40808809e-03  & 6.06422458e-03  & 6.53074915e-03  \\ 
  &   &   & 2.49393016e-04  & 4.76270304e-04  & 6.47896649e-04  & 7.80311455e-04  \\ 
  &   &   &   & 1.93957821e-05  & 4.23377364e-05  & 6.37060750e-05  \\ 
  &   &   &   &   & 1.29097658e-06  & 3.21558780e-06  \\ 
  &   &   &   &   &   & 7.63259101e-08  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal third order explicit RK methods for $s=[4, 5, 6, 7, 8, 9]$}
\label{tbl:stab-coeffs-optimal-erk3-0}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk3-1.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 10 & 11 & 12 & 13 & 14 & 15 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 3.94666993e-02  & 3.98703694e-02  & 4.01841546e-02  & 4.04193375e-02  & 4.05874510e-02  & 4.07390664e-02  \\ 
  & 6.86287348e-03  & 7.11608836e-03  & 7.31536299e-03  & 7.46754424e-03  & 7.58171078e-03  & 7.68169372e-03  \\ 
  & 8.81078156e-04  & 9.60578268e-04  & 1.02463837e-03  & 1.07525471e-03  & 1.11454390e-03  & 1.14872728e-03  \\ 
  & 8.20947814e-05  & 9.76500363e-05  & 1.10802924e-04  & 1.21710887e-04  & 1.30520195e-04  & 1.38257479e-04  \\ 
  & 5.29763422e-06  & 7.30574829e-06  & 9.15553685e-06  & 1.08010779e-05  & 1.22040261e-05  & 1.34694736e-05  \\ 
  & 2.13383191e-07  & 3.82396198e-07  & 5.62659834e-07  & 7.40783735e-07  & 9.04936047e-07  & 1.06021157e-06  \\ 
  & 4.06700109e-09  & 1.25868238e-08  & 2.43798908e-08  & 3.81123776e-08  & 5.23058876e-08  & 6.67788902e-08  \\ 
  &   & 1.97183637e-10  & 6.68096225e-10  & 1.39154611e-09  & 2.28279356e-09  & 3.30181795e-09  \\ 
  &   &   & 8.74959885e-12  & 3.22943935e-11  & 7.10547606e-11  & 1.23952338e-10  \\ 
  &   &   &   & 3.59576777e-13  & 1.41106464e-12  & 3.33327720e-12  \\ 
  &   &   &   &   & 1.34819787e-14  & 5.73869048e-14  \\ 
  &   &   &   &   &   & 4.76607053e-16  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal third order explicit RK methods for $s=[10, 11, 12, 13, 14, 15]$}
\label{tbl:stab-coeffs-optimal-erk3-1}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk3-2.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l} 
 & \multicolumn{5}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 16 & 17 & 18 & 19 & 20 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 4.08638452e-02  & 4.09555209e-02  & 4.10392610e-02  & 4.11054681e-02  & 4.11643252e-02  \\ 
  & 7.76424281e-03  & 7.82775817e-03  & 7.88465616e-03  & 7.93051751e-03  & 7.97108714e-03  \\ 
  & 1.17733578e-03  & 1.20005481e-03  & 1.22022863e-03  & 1.23687831e-03  & 1.25153543e-03  \\ 
  & 1.44873500e-04  & 1.50287923e-04  & 1.55099805e-04  & 1.59167279e-04  & 1.62750797e-04  \\ 
  & 1.45856163e-05  & 1.55302057e-05  & 1.63788564e-05  & 1.71148216e-05  & 1.77682773e-05  \\ 
  & 1.20327979e-06  & 1.32944976e-06  & 1.44529196e-06  & 1.54876647e-06  & 1.64206559e-06  \\ 
  & 8.09588363e-08  & 9.41468854e-08  & 1.06676374e-07  & 1.18279595e-07  & 1.28994293e-07  \\ 
  & 4.39094848e-09  & 5.47804945e-09  & 6.56322461e-09  & 7.61507423e-09  & 8.61960818e-09  \\ 
  & 1.88042297e-10  & 2.58464130e-10  & 3.33799236e-10  & 4.11247737e-10  & 4.88654863e-10  \\ 
  & 6.14293394e-12  & 9.67428098e-12  & 1.38336561e-11  & 1.84531837e-11  & 2.33578881e-11  \\ 
  & 1.44297526e-13  & 2.77261928e-13  & 4.56635182e-13  & 6.77556986e-13  & 9.31671924e-13  \\ 
  & 2.17678753e-15  & 5.73082515e-15  & 1.15792084e-14  & 1.98842864e-14  & 3.05174416e-14  \\ 
  & 1.58823582e-17  & 7.62478901e-17  & 2.12330658e-16  & 4.49580486e-16  & 8.01346278e-16  \\ 
  &   & 4.91531676e-19  & 2.51179855e-18  & 7.36852620e-18  & 1.62523070e-17  \\ 
  &   &   & 1.44224648e-20  & 7.80687552e-20  & 2.39441875e-19  \\ 
  &   &   &   & 4.02166753e-22  & 2.28441243e-21  \\ 
  &   &   &   &   & 1.06125958e-23  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal thirdorder RK methods for $s=[16, 17, 18, 19, 20]$}
\label{tbl:stab-coeffs-optimal-erk3-2}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk4-0.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 5 & 6 & 7 & 8 & 9 & 10 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 4e-02  & 4e-02  & 4e-02  & 4e-02  & 4e-02  & 4e-02  \\ 
  & 5.15766348e-03  & 6.83418417e-03  & 7.37565694e-03  & 7.65804482e-03  & 7.82693112e-03  & 7.93815939e-03  \\ 
  &   & 5.29792706e-04  & 8.17425058e-04  & 9.78109514e-04  & 1.07711274e-03  & 1.14331481e-03  \\ 
  &   &   & 4.22060440e-05  & 7.74502671e-05  & 1.02767717e-04  & 1.21031664e-04  \\ 
  &   &   &   & 2.85920385e-06  & 6.08431065e-06  & 8.91021065e-06  \\ 
  &   &   &   &   & 1.68650440e-07  & 4.08468389e-07  \\ 
  &   &   &   &   &   & 8.79826993e-09  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal fourth order explicit RK methods for $s=[5, 6, 7, 8, 9, 10]$}
\label{tbl:stab-coeffs-optimal-erk4-0}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk4-1.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 11 & 12 & 13 & 14 & 15 & 16 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 4e-02  & 4e-02  & 4e-02  & 4e-02  & 4e-02  & 4e-02  \\ 
  & 8.01644431e-03  & 8.06999615e-03  & 8.11437744e-03  & 8.14358401e-03  & 8.16799843e-03  & 8.19096887e-03  \\ 
  & 1.19028637e-03  & 1.22326650e-03  & 1.25007619e-03  & 1.26866146e-03  & 1.28392230e-03  & 1.29794141e-03  \\ 
  & 1.34620265e-04  & 1.44592616e-04  & 1.52744376e-04  & 1.58664465e-04  & 1.63544624e-04  & 1.67950007e-04  \\ 
  & 1.12560645e-05  & 1.31182562e-05  & 1.46954572e-05  & 1.59058224e-05  & 1.69250580e-05  & 1.78422705e-05  \\ 
  & 6.57937455e-07  & 8.85429046e-07  & 1.09354463e-06  & 1.26583783e-06  & 1.41706539e-06  & 1.55527318e-06  \\ 
  & 2.40663162e-08  & 4.20057804e-08  & 6.09237412e-08  & 7.84338426e-08  & 9.48948149e-08  & 1.10531334e-07  \\ 
  & 4.15542093e-10  & 1.25297041e-09  & 2.39849399e-09  & 3.65841060e-09  & 4.97842890e-09  & 6.32185713e-09  \\ 
  &   & 1.77169187e-11  & 5.96431259e-11  & 1.21135545e-10  & 1.97646304e-10  & 2.84702601e-10  \\ 
  &   &   & 7.05881952e-13  & 2.54346580e-12  & 5.59559299e-12  & 9.74307675e-12  \\ 
  &   &   &   & 2.55041129e-14  & 1.00857704e-13  & 2.38604991e-13  \\ 
  &   &   &   &   & 8.71289522e-16  & 3.73129529e-15  \\ 
  &   &   &   &   &   & 2.80380426e-17  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal fourth order explicit RK methods for $s=[11, 12, 13, 14, 15, 16]$}
\label{tbl:stab-coeffs-optimal-erk4-1}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk4-2.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l} 
 & \multicolumn{4}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 17 & 18 & 19 & 20 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 4e-02  & 4e-02  & 4e-02  & 4e-02  \\ 
  & 8.20563908e-03  & 8.22246230e-03  & 8.23362078e-03  & 8.24182409e-03  \\ 
  & 1.30746673e-03  & 1.31762357e-03  & 1.32474213e-03  & 1.33021276e-03  \\ 
  & 1.71106269e-04  & 1.74317919e-04  & 1.76675406e-04  & 1.78542904e-04  \\ 
  & 1.85334676e-05  & 1.92182281e-05  & 1.97420818e-05  & 2.01683553e-05  \\ 
  & 1.66511655e-06  & 1.77299446e-06  & 1.85900070e-06  & 1.93092851e-06  \\ 
  & 1.23746015e-07  & 1.36844783e-07  & 1.47771712e-07  & 1.57197089e-07  \\ 
  & 7.54703097e-09  & 8.79701784e-09  & 9.89672954e-09  & 1.08814654e-08  \\ 
  & 3.72413807e-10  & 4.66698018e-10  & 5.55259836e-10  & 6.38383926e-10  \\ 
  & 1.45339408e-11  & 2.01257404e-11  & 2.58346558e-11  & 3.15282812e-11  \\ 
  & 4.32602924e-13  & 6.89055312e-13  & 9.81118280e-13  & 1.29655347e-12  \\ 
  & 9.24242589e-15  & 1.80517195e-14  & 2.96882769e-14  & 4.36698010e-14  \\ 
  & 1.26399516e-16  & 3.40387653e-16  & 6.89587251e-16  & 1.17536958e-15  \\ 
  & 8.32237604e-19  & 4.11829526e-18  & 1.15619357e-17  & 2.43429032e-17  \\ 
  &   & 2.40373663e-20  & 1.24714765e-19  & 3.64673221e-19  \\ 
  &   &   & 6.50638355e-22  & 3.52066594e-21  \\ 
  &   &   &   & 1.64616635e-23  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal fourthorder RK methods for $s=[17, 18, 19, 20]$}
\label{tbl:stab-coeffs-optimal-erk4-2}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk5-0.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 7 & 8 & 9 & 10 & 11 & 12 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 4e-02  & 4e-02  & 4e-02  & 4e-02  & 4e-02  & 4e-02  \\ 
  & 8e-03  & 8e-03  & 8e-03  & 8e-03  & 8e-03  & 8e-03  \\ 
  & 1.26199602e-03  & 1.34402290e-03  & 1.37249276e-03  & 1.38337256e-03  & 1.38700474e-03  & 1.38823591e-03  \\ 
  & 1.01581682e-04  & 1.54629263e-04  & 1.78076081e-04  & 1.88855902e-04  & 1.93668657e-04  & 1.95903109e-04  \\ 
  &   & 8.94209847e-06  & 1.56824699e-05  & 1.96783351e-05  & 2.18746355e-05  & 2.30707280e-05  \\ 
  &   &   & 6.73079335e-07  & 1.34961235e-06  & 1.84045849e-06  & 2.16019147e-06  \\ 
  &   &   &   & 4.45182842e-08  & 1.00331484e-07  & 1.48382983e-07  \\ 
  &   &   &   &   & 2.61817522e-09  & 6.55461940e-09  \\ 
  &   &   &   &   &   & 1.38488099e-10  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal fifth order explicit RK methods for $s=[7, 8, 9, 10, 11, 12]$}
\label{tbl:stab-coeffs-optimal-erk5-0}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk5-1.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l|l|l} 
 & \multicolumn{6}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 13 & 14 & 15 & 16 & 17 & 18 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 4e-02  & 4e-02  & 4e-02  & 4e-02  & 4e-02  & 4e-02  \\ 
  & 8e-03  & 8e-03  & 8e-03  & 8e-03  & 8e-03  & 8e-03  \\ 
  & 1.38573329e-03  & 1.38385545e-03  & 1.38355928e-03  & 1.38432033e-03  & 1.38520514e-03  & 1.38597885e-03  \\ 
  & 1.95543282e-04  & 1.94987578e-04  & 1.95010638e-04  & 1.95504364e-04  & 1.96038869e-04  & 1.96507209e-04  \\ 
  & 2.33517397e-05  & 2.34037434e-05  & 2.35203327e-05  & 2.37238121e-05  & 2.39215380e-05  & 2.40900960e-05  \\ 
  & 2.29603873e-06  & 2.35856980e-06  & 2.41185944e-06  & 2.47030127e-06  & 2.52273423e-06  & 2.56637481e-06  \\ 
  & 1.76850782e-07  & 1.93448147e-07  & 2.06221064e-07  & 2.18098610e-07  & 2.28384785e-07  & 2.36891641e-07  \\ 
  & 9.90059509e-09  & 1.23169694e-08  & 1.42508447e-08  & 1.59838368e-08  & 1.74948324e-08  & 1.87649311e-08  \\ 
  & 3.55376564e-10  & 5.67378692e-10  & 7.61135135e-10  & 9.43263295e-10  & 1.10995352e-09  & 1.25615177e-09  \\ 
  & 6.10865239e-12  & 1.67439687e-11  & 2.93697479e-11  & 4.29407091e-11  & 5.66346766e-11  & 6.95763080e-11  \\ 
  &   & 2.37013826e-13  & 7.26727258e-13  & 1.41199608e-12  & 2.22925825e-12  & 3.09854967e-12  \\ 
  &   &   & 8.64676521e-15  & 2.98036310e-14  & 6.34530781e-14  & 1.06505616e-13  \\ 
  &   &   &   & 3.03021333e-16  & 1.16149792e-15  & 2.65005471e-15  \\ 
  &   &   &   &   & 1.02642197e-17  & 4.24629121e-17  \\ 
  &   &   &   &   &   & 3.28982072e-19  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal fifth order explicit RK methods for $s=[13, 14, 15, 16, 17, 18]$}
\label{tbl:stab-coeffs-optimal-erk5-1}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-optimal-erk5-2.tex <==
\begin{sidewaystable}[htbp!]
\centering
\begin{tabular}{l|l|l|l|l} 
 & \multicolumn{4}{c}{Monomial basis coefficients} \\ \hline 
$s$ & 19 & 20 & 21 & 22 \\ \hline 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 1e+00  & 1e+00  & 1e+00  & 1e+00  \\ 
  & 5e-01  & 5e-01  & 5e-01  & 5e-01  \\ 
  & 2e-01  & 2e-01  & 2e-01  & 2e-01  \\ 
  & 4e-02  & 4e-02  & 4e-02  & 4e-02  \\ 
  & 8e-03  & 8e-03  & 8e-03  & 8e-03  \\ 
  & 1.38664176e-03  & 1.38715961e-03  & 1.38755060e-03  & 1.38784225e-03  \\ 
  & 1.96910466e-04  & 1.97230266e-04  & 1.97477588e-04  & 1.97666123e-04  \\ 
  & 2.42334553e-05  & 2.43486790e-05  & 2.44387876e-05  & 2.45086094e-05  \\ 
  & 2.60302432e-06  & 2.63278930e-06  & 2.65627917e-06  & 2.67473835e-06  \\ 
  & 2.44020894e-07  & 2.49889344e-07  & 2.54580778e-07  & 2.58324745e-07  \\ 
  & 1.98440188e-08  & 2.07514508e-08  & 2.14915461e-08  & 2.20939985e-08  \\ 
  & 1.38450022e-09  & 1.49606096e-09  & 1.58978382e-09  & 1.66813437e-09  \\ 
  & 8.15921267e-11  & 9.25569101e-11  & 1.02161928e-10  & 1.10483112e-10  \\ 
  & 3.97814878e-12  & 4.83834956e-12  & 5.63640465e-12  & 6.36129836e-12  \\ 
  & 1.56018582e-13  & 2.09391414e-13  & 2.62919799e-13  & 3.14674131e-13  \\ 
  & 4.72689318e-15  & 7.29711617e-15  & 1.01629893e-14  & 1.31722730e-14  \\ 
  & 1.03792934e-16  & 1.96721522e-16  & 3.16716712e-16  & 4.57403117e-16  \\ 
  & 1.46969380e-18  & 3.84976440e-18  & 7.64603469e-18  & 1.28209045e-17  \\ 
  & 1.00764422e-20  & 4.86644768e-20  & 1.34197696e-19  & 2.78757420e-19  \\ 
  &   & 2.98364943e-22  & 1.52383405e-21  & 4.41235330e-21  \\ 
  &   &   & 8.40580879e-24  & 4.52476621e-23  \\ 
  &   &   &   & 2.25719772e-25  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the optimal fifthorder RK methods for $s=[19, 20, 21, 22]$}
\label{tbl:stab-coeffs-optimal-erk5-2}
\end{sidewaystable} 


==> tables/stab_poly_coeffs/table-stab-coeffs-selected-optimal-erk2.tex <==
\begin{table}[htbp!]
\centering
\begin{tabular}{l|l|l} 
 & \multicolumn{2}{c}{Monomial basis coefficients $(\beta_j)$} \\ \hline 
$s$ & 3                     & 8 \\ \hline 
  & 1                       & 1  \\ 
  & 1                       & 1  \\ 
  & 1/2                     & 1/2  \\ 
  & 9.0728994733419860e-02  & 1.5537269246963092e-01  \\ 
  &                         & 3.2481270611740019e-02  \\ 
  &                         & 4.6452162970027997e-03  \\ 
  &                         & 4.4302275455858066e-04  \\ 
  &                         & 2.5797693971775763e-05  \\ 
  &                         & 7.0797555384137189e-07  \\ 
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the selected optimal second-order explicit Runge--Kutta methods.}
\label{tab:stab-coeffs-selected-optimal-erk2}
\end{table}  


==> tables/stab_poly_coeffs/table-stab-coeffs-selected-optimal-erk3.tex <==
\begin{table}[htbp!]
\centering
\begin{tabular}{l|l|l} 
 & \multicolumn{2}{c}{Monomial basis coefficients ($\beta_j$)} \\ \hline 
$s$ & 5                        & 17     \\ \hline 
    & 1                        & 1  \\ 
    & 1                        & 1   \\ 
    & 1/2                      & 1/2   \\ 
    & 1/6                      & 1/6   \\ 
    & 3.1737676985346464e-02   & 4.0955520938708016e-02  \\ 
    & 2.7477333443275062e-03   & 7.8277581714590247e-03  \\ 
    &                          & 1.2000548060924175e-03 \\ 
    &                          & 1.5028792258720729e-04 \\ 
    &                          & 1.5530205680353078e-05 \\ 
    &                          & 1.3294497556515817e-06 \\
    &                          & 9.4146885376481696e-08 \\
    &                          & 5.4780494452233359e-09\\
    &                          & 2.5846413034579029e-10\\
    &                          & 9.6742809810714128e-12\\
    &                          & 2.7726192829265364e-13\\
    &                          & 5.7308251483600546e-15\\
    &                          & 7.6247890055814194e-17\\
    &                          & 4.9153167585702277e-19\\
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the selected optimal third-order explicit Runge--Kutta methods.}
\label{tab:stab-coeffs-selected-optimal-erk3}
\end{table} 


==> tables/stab_poly_coeffs/table-stab-coeffs-selected-optimal-erk4.tex <==
\begin{table}[htbp!]
\centering
\begin{tabular}{l|l|l} 
 & \multicolumn{2}{c}{Monomial basis coefficients ($\beta_j$)} \\ \hline 
$s$ & 9                       & 18 \\ \hline 
    & 1                       & 1  \\ 
    & 1                       & 1  \\ 
    & 1/2                     & 1/2  \\ 
    & 1/6                     & 1/6  \\ 
    & 1/24                    & 1/24  \\ 
    & 7.8269311157401159e-03  & 8.2224623040129657e-03  \\ 
    & 1.0771127377147780e-03  & 1.3176235681504832e-03  \\ 
    & 1.0276771730475306e-04  & 1.7431791851035765e-04  \\ 
    & 6.0843106462582707e-06  & 1.9218228071467922e-05  \\ 
    & 1.6865044017806091e-07  & 1.7729944633853745e-06  \\ 
    &                         & 1.3684478313698141e-07  \\ 
    &                         & 8.7970178374215285e-09  \\
    &                         & 4.6669801804917137e-10  \\
    &                         & 2.0125740364966102e-11  \\
    &                         & 6.8905531222694872e-13  \\
    &                         & 1.8051719499410950e-14  \\
    &                         & 3.4038765308454378e-16  \\
    &                         & 4.1182952611782795e-18  \\
    &                         & 2.4037366335443982e-20  \\
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the selected optimal fourth-order explicit Runge--Kutta methods.}
\label{tab:stab-coeffs-selected-optimal-erk4}
\end{table} 


==> tables/stab_poly_coeffs/table-stab-coeffs-selected-optimal-erk5.tex <==
\begin{table}[htbp!]
\centering
\begin{tabular}{l|l|l} 
 & \multicolumn{2}{c}{Monomial basis coefficients ($\beta_j$)} \\ \hline 
$s$ & 10                        & 20 \\ \hline 
    & 1                         & 1  \\ 
    & 1                         & 1  \\ 
    & 1/2                       & 1/2  \\ 
    & 1/6                       & 1/6  \\ 
    & 1/24                      & 1/24  \\ 
    & 1/20                      & 1/120  \\ 
    & 1.3833725557698888e-03    & 1.3871596079307906e-03 \\ 
    & 1.8885590169131643e-04    & 1.9723026648287164e-04  \\ 
    & 1.9678335130137695e-05    & 2.4348678983779023e-05  \\ 
    & 1.3496123473091492e-06    & 2.6327892962607919e-06  \\ 
    & 4.4518284180652831e-08    & 2.4988934365384683e-07 \\ 
    &                           & 2.0751450841667420e-08 \\ 
    &                           & 1.4960609591038679e-09 \\
    &                           & 9.2556910065861905e-11 \\
    &                           & 4.8383495584594970e-12 \\
    &                           & 2.0939141375052135e-13 \\
    &                           & 7.2971161737676861e-15 \\
    &                           & 1.9672152192631305e-16 \\
    &                           & 3.8497644019093262e-18 \\
    &                           & 4.8664476802682760e-20 \\
    &                           & 2.9836494323104484e-22 \\
 \hline 
\end{tabular} 
\caption{Stability polynomial coefficients of the selected optimal fifth-order explicit Runge--Kutta methods.}
\label{tab:stab-coeffs-selected-optimal-erk5}
\end{table} 

